StRegA: Unsupervised Anomaly Detection in Brain MRIs using a Compact Context-encoding Variational Autoencoder

Expert interpretation of anatomical images of the human brain is the central part of neuro-radiology. Several machine learning-based techniques have been proposed to assist in the analysis process. However, the ML models typically need to be trained to perform a specific task, e.g., brain tumour segmentation or classification. Not only do the corresponding training data require laborious manual annotations, but a wide variety of abnormalities can be present in a human brain MRI - even more than one simultaneously, which renders representation of all possible anomalies very challenging. Hence, a possible solution is an unsupervised anomaly detection (UAD) system that can learn a data distribution from an unlabelled dataset of healthy subjects and then be applied to detect out of distribution samples. Such a technique can then be used to detect anomalies - lesions or abnormalities, for example, brain tumours, without explicitly training the model for that specific pathology. Several Variational Autoencoder (VAE) based techniques have been proposed in the past for this task. Even though they perform very well on controlled artificially simulated anomalies, many of them perform poorly while detecting anomalies in clinical data. This research proposes a compact version of the "context-encoding" VAE (ceVAE) model, combined with pre and post-processing steps, creating a UAD pipeline (StRegA), which is more robust on clinical data, and shows its applicability in detecting anomalies such as tumours in brain MRIs. The proposed pipeline achieved a Dice score of 0.642$\pm$0.101 while detecting tumours in T2w images of the BraTS dataset and 0.859$\pm$0.112 while detecting artificially induced anomalies, while the best performing baseline achieved 0.522$\pm$0.135 and 0.783$\pm$0.111, respectively.

==> figs/titlepage.tex <==
\begin{titlepage}
  \thispagestyle{titlepage}
  \begin{center}
  {\LARGE \myuniversity}\\[5mm]
  \begin{figure*}[h]
   \hbox{}\hfill
   \begin{minipage}[t]{9cm}
			 \centering
			 \includegraphics[width=7cm]{logos/OVGU_SIGN_druck.eps}
   \end{minipage}
   \hfill\hbox{}
  \end{figure*}
  {\large \myschool\\ \mydepartment}\\[10mm]
 % {\LARGE \kindOfThesis}\\[10mm]
		%{\large\bf \titleOfThesis}\\[10mm]
  {\Large\bf \titleOfThesis}\\[10mm]
  {\small Authors:}\\[1mm]
  {\large \myfirstname}\\[5mm]
  {\small \myschool} \\[1mm]
  {\small \myuni} \\[1mm]
  {\small \today}\\[15mm]
  
  \vspace{3cm}
  \renewcommand{\arraystretch}{.5}
  \begin{tabular}{ccc}
	{\large \firstadvisor}\textsuperscript{1,2,3} & {\large \secondadvisor}\textsuperscript{1,4} & {\large \thirdadvisor}\textsuperscript{3,4} \\
	{\small 1st Advisor} & {\small 2nd Advisor}  & {\small 3rd Advisor}\\[2mm]
	{\large \firstexaminar}\textsuperscript{4,5,6} & {\large \secondexaminar} \textsuperscript{1,5,6,7}& {\large \thirdexaminar}\textsuperscript{2,3,6} \\
	{\small 1st Examiner} & {\small 2nd Examiner}  & {\small 3rd Examiner}\\[2mm]
    \multicolumn{3}{l}{\small \textsuperscript{1}Department of Biomedical Magnetic Resonance,Otto von Guericke  University, Magdeburg, Germany} \\
    \multicolumn{3}{l}{\small \textsuperscript{2}  Data and Knowledge Engineering Group, Otto von Guericke University, Magdeburg, Germany} \\[0.5mm]
    \multicolumn{3}{l}{\small \textsuperscript{3} Faculty of Computer Science, Otto von Guericke University, Magdeburg, Germany} \\[0.5mm]
    \multicolumn{3}{l}{\small \textsuperscript{4} MedDigit, Department of Neurology, Medical Faculty, University Hospital, Magdeburg, Germany} \\[0.5mm] 
    \multicolumn{3}{l}{\small \textsuperscript{5}German Centre for Neurodegenerative Diseases, Magdeburg, Germany} \\[0.5mm]
    \multicolumn{3}{l}{\small \textsuperscript{6} Center for Behavioral Brain Sciences, Magdeburg, Germany} \\[0.5mm]
    \multicolumn{3}{l}{\small \textsuperscript{7}Leibniz Institute for Neurobiology, Magdeburg, Germany} \\[0.5mm]
  \end{tabular}
  
		\renewcommand{\arraystretch}{1}
  \end{center}
\end{titlepage}

\thispagestyle{empty}

\cleardoublepage

% =============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Inhaltsverzeichnis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\setcounter{tocdepth}{2}
\tableofcontents

%\addcontentsline{toc}{chapter}{Abbildungsverzeichnis}
%\listoffigures

%\addcontentsline{toc}{chapter}{Tabellenverzeichnis}
%\listoftables

%\addcontentsline{toc}{chapter}{Algorithmenverzeichnis}
%\listofalgorithms
%\todo{Anleitung Algorithmen schreiben: \url{http://en.wikibooks.org/wiki/LaTeX/Algorithms}}

\cleardoublepage
% =============================================================================

\phantomsection
\section*{Abstract}
\addcontentsline{toc}{chapter}{Abstract}
This report illustrates a pipeline called StRegA : Segmentation Regularised Anomaly to achieve Unsupervised anomaly detection in MRI images. Manual analysis of volumetric data Magnetic Resonance (MR) is mainly performed to identify irregularities or investigate symptoms to neurological causes. If applied to solve existing problems this automated approach would help in reducing the time, possibility of error and pre-existing large amounts of data. Many studies point out that up to 5-10 \%  of pathologies are misjudged. 

In the last decade, the efficacy of machine learning based automated methods for this task has been getting better and has seen significant advancement in the algorithms used. Furthermore, these scientific results display abilities on par with experts. Of course, requiring large amounts of data for supervised learning is difficult because of the cost requirements and availability of such data. Our approach orients towards research on overcoming these difficulties and utilise annotation-free unsupervised methods.

Our model unlike supervised approaches is also not pathology-specific and the distributional outliers can now be recognised as anomalies. Our framework involves simplifying the data distribution and the model layers to have better latent representation. This allowed reconstruction without out of distribution anomalies. We benchmarked that with existing approaches that are currently popular. This report showcases the approach applied to Brain MRI images however the pipeline concept can be positively translated to other imaging modalities, which further opens opportunities to explore and integrate machine learning into radiology.


\cleardoublepage
% =============================================================================


==> sections/0_intro.tex <==
\section{Introduction}
\label{sec:intro}
Acquiring and analysing magnetic resonance images (MRIs) is an integral part of the work of neuroradiologists. MRI is free from harmful ionising radiation and its ability to show excellent soft-tissue contrast, making it the preferred imaging modality for brain imaging in clinical practice~\citep{hagens2019impact}. MR images are used to examine numerous brain pathologies, and manually analysing or annotating such images is part of the radiologists’ regular duties. Not only such duties are time-consuming and laborious, but they are also error-prone~\citep{brady2017error}. Noting from \citet{bruno2015understanding}, diagnostics of brain pathology remain undiscovered in up to 5-10 \% of cases. The medical image analysis community has made numerous contributions toward automating specific steps, focusing on human-level accuracy at economically adequate computational complexity. With advancements in artificial intelligence, outstanding achievements have been marked in the detection and segmentation of lesions. Furthermore, these scientific results display abilities on par with experts \citep{menze2014multimodal}. Such automated methods try to assist the radiologists in the decision-making process - reducing the workload and observer dependency while improving the workflow and diagnostic accuracy \citep{guerrero2018white}. 

Most of these automatic methods are based on supervised learning techniques, relying on the quality and quantity of labelled data. They utilise a vast amount of annotated training data  -  ranging from thousands to millions of samples. These trained models are usually specialists in dealing with domain-specific tasks or the tasks they have been optimised for - which can also be considered as the bottleneck in such a method as they typically follow a ‘focus point solution’ design, which means they are often very focused on one type of pathology or lesion. Considering an example of cerebral small vessel disease, supervised solutions are challenging to develop since the damage is complex in terms of lesion size, contrast, or morphology~\citep{wardlaw2013neuroimaging}. Considering the complex field of medicine, procuring annotated data is a tedious manual process - while it might be challenging to annotate concerning all the possible pathologies.  

An alternative solution to the conventional approach of the supervised machine learning method to detect brain pathologies is an unsupervised anomaly detection (UAD) system. Anomaly detection is an approach that distinguishes anomalies completely based on characteristics that describe regular data. Since the feature of possible irregularities is not learned, they stand from the normal distribution and can be consequently detected. Anomaly detection solutions are useful in cases where anomalies are to be detected, but their manifestation is not known, and they even might occur very rarely - making it difficult to create a large dataset for supervised training~\citep{pimentel2014review}. Anomaly detection techniques have been applied for multiple tasks, including credit card fraud detection \citep{phua2004minority}, aerospace monitoring during flight \citep{clifton2007framework}, illegal object detection at airports \citep{akcay2018ganomaly} or detecting faulty microprocessors \citep{kim2012machine}.

Anomaly detection in medical imaging is defined as identifying relevant indicators of diseases and differentiating them from those of typical healthy tissue characteristics. UAD systems can directly learn the data distribution from a large cohort of un-annotated healthy subjects to detect out-of-distribution or anomalous samples to identify cases for further inspection. As anomaly detection does not depend on reference annotations, this approach does not require any human input and can therefore be used to identify any medical condition. Unsupervised segmentation of brain regions for anomaly detection is clinically relevant as it can assist radiologists. It is also of great interest to the medical image analysis community as it eliminates the need for pixel-level annotations, which is an expensive process and is often a prerequisite for supervised training of the networks. However, it is worth mentioning that a system, such as UAD, does not differentiate between different types of anomalies, i.e. lesions and artefacts - both will be treated as anomalies by a UAD system. Variational autoencoders (VAEs) are one of the most commonly used techniques for anomaly detection, along with methods based on Generative Adversarial Networks (GANs)~\citep{zimmerer2019unsupervised,liu2020using,garcia2021usage,pinaya2022unsupervised}. However, many of such techniques fail to perform well when it comes to real clinical data. This research aims to extend the research field of anomaly detection by creating a UAD pipeline capable of working with clinical data for the detection of clinically-relevant anomalies (e.g. lesions) and evaluating its performance for the task of brain tumour detection. 

==> sections/1_relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}
Auto-encoders are trained by minimising its reconstruction error~\citep{alain2014regularized}. Different types of reconstruction errors are commonly used in unsupervised anomaly detection, acknowledging that regular distribution models cannot effectively reproduce anomalies~\citep{ribeiro2018study}. Therefore, regular anomaly-free data is distinguishable from anomalous data with the degree of error differences in terms of reconstruction. The majority of the methods assume reconstruction errors (losses) are optimised for average distribution data, whereas anomalies are impacted with significant losses when their dimensions are reduced. 

Generative Adversarial Networks (GANs)~\citep{goodfellow2014generative} and Variational Autoencoder (VAEs) \citep{kingma2013auto}  are two essential methods based on latent space information modelling, and they have been employed for the task of anomaly detection~\citep{xu2018unsupervised,yan2020unsupervised}. However, both these methods have different approaches for modelling the distribution. VAE  applies variational inference to approximate the data distribution. The posterior distribution is encoded into latent space using the encoder network of the VAE, whereas the decoder network is responsible for modelling the likelihood. Unlike VAE, the generator network of the GAN transforms the prior distribution of the random samples in the latent space into data samples that an optimised classifier cannot distinguish. The obtained data distribution is inferable, and GAN is mainly a sampler. Recently some researchers \citep{carrara2021combining} have coupled an autoencoder with GAN to derive enhanced latent representations in the domain of anomaly detection. 

On the other hand, after revolutionising the field of natural language processing, Transformers~\citep{vaswani2017attention} have found applications in other areas such as computer vision, including modelling brain images with impressive results. The defining characteristic of a transformer is that it relies on attention mechanisms to capture
interactions between inputs, regardless of their relative position to one another. The output is computed as a weighted sum of the values, where the weight assigned to each value is computed by a compatibility function of the query with the corresponding key. Transformers have been used to model brain images for the purpose of anomaly detection after assuming an arbitrary ordering to transform the latent discrete variables $z_q$ into a 1D sequence s and training the transformer to maximise the training data’s log-likelihood in an autoregressive fashion~\citep{pinaya2022unsupervised}. However, such methods are typically memory-hungry - making them difficult to use with limited computing resources. VAEs can be less computationally expensive than transformers, making them more suitable for using them widely. Hence, this paper focuses is on VAE-based techniques and some of the related AE and VAE based works which were studied and  experimented with for baseline selection, are discussed in detail.

\subsection{Adversarial Autoencoder}
\label{sec:AdvAE}
Autoencoders~\citep{rumelhart1985learning,kramer1991nonlinear} try to learn an underlying function - which is an approximation to the identity function - trying to reproduce the input as its output, learning a latent space representation (LSR) of the input in the process~\citep{ng2011sparse}. The model's output is compared against the input with the help of reconstruction loss, which is then backpropagated to train the network. Adversarial autoencoder \citep{makhzani2016adversarial} converts an autoencoder into a generative model, which has also been used for the task of anomaly detection \citep{beggel2019robust,li2019video}. The objective is two-fold - a regular reconstruction loss and an adversarial training loss. The second loss criterion tends to match the aggregated posterior distribution of the latent space of the autoencoder to an arbitrary prior distribution. An outcome of this architecture bounds the encoder module to learn the data distribution close to the prior distribution, and the decoder maps the imposed prior to the data distribution. The encoding function of the encoder is formally represented as 
\begin{equation} 
q(z) = \int_x q(z\mid x) p_d(x) dx 
\end{equation} 
where $x$ is the input and $z$ is its latent representation vector. $p(z)$ be the prior distribution to be imposed on the latent vectors, $q(z|x)$ is an encoding dimension, and p(x$\mid$ z) is the decoding distribution. Also, $p_d(x)$ is the data distribution and $p(x)$ is the model distribution. The adversarial autoencoder is regularised by matching this aggregated posterior $q(z)$ to an arbitrary prior, $p(z)$. The whole training takes place in two phases - \emph{reconstruction} phase where the encoder and decoder are updated to minimise the reconstruction error in the input. Later in the \emph{regularisation} phase, the adversarial network updates the discriminator to classify better actual samples (from the prior) from the generated samples (from the encoder). Finally, the generator or the encoder is updated to confuse the discriminator. 

\subsection{Scale-Space Autoencoder}
\label{sec:ssAE}
Many variations of autoencoders have been proposed. One of them is  Scale-Space Autoencoder (SSAE) \citep{baur2020scalespace}.This framework is used for unsupervised anomaly detection based on the Laplacian pyramid, allowing efficient compression and reconstruction of brain MRI images with high fidelity and successfully suppressing anomalies. Contrary to other frameworks, the SSAE framework models the distribution of the scale-space representation of healthy brain MRI. The Laplacian pyramid is a multi-scale representation of the input image; it allows efficient segmentation of anomalies at different resolutions and then aggregates the results. SSAE architecture is an encoder-decoder network that aims to localise anomalies from reconstruction residuals. The frequency band of the input data is split by compressing and reconstructing the Laplacian pyramid of the healthy brain MRI. The input image $x$ is repeatedly smoothed and downsampled to obtain a Laplacian pyramid with K levels. Reconstruction can be recursively determined using
\begin{equation}
   \hat{x} = \sum_{k=0}^{K-1} u(I_{K-k}) + H_{K-1-k}
\end{equation}
where $I_k$ is the low-resolution representation of the image x after K down samplings and high-frequency residuals $H_0,..,H_{K-1}$ which are obtained at each level k using :
\begin{equation}
   H_k = I_k - u(I_{k+1}) ; \forall 0	\leq k<K
\end{equation}
The overall loss can be defined as the weighted sum of losses at all scales:
\begin{equation}
   L = \sum_{k=0}^{K} \lambda_kL_k
\end{equation}
where,
\begin{equation}
   L_k = l2_{norm}(I_k, \hat{I_k}) = l2(I_k, u(\hat{I_k}+\hat{H_k})
\end{equation}


\subsection{Bayesian Skip autoencoder}
\label{sec:SkipAE}
Bayesian Skip autoencoder  \citep{cccc}  is formulated on a concept that has been used and proven advantageous for biomedical image segmentation. This framework makes use of skip connections that allow the models with limited capacity to be trained and utilised for unsupervised anomaly detection. Skip connections in autoencoders facilitate the reconstruction of high-resolution and complex medical data with high fidelity. A drop-out-based identity mitigation technique is employed to prevent the model from learning an identity mapping and allowing it to bypass the lower levels of the autoencoder. The loss function for the model can be defined as:
 \begin{equation}
   L(x, \hat{x}) = L1(x, \hat{x}) - gdl(x, \hat{x})
\end{equation}
Here, $L1$  is defined as the L1 Manhattan distance between the input and its reconstruction $x$ and $\hat{x}$ respectively, $gdl(.,.)$ is the gradient difference loss.

\subsection{Variational Autoencoder (VAE)}
\label{sec:VAE}
Variational autoencoders (VAEs)~\citep{kingma2013auto} belong to a class of generative models that provides a probabilistic way to represent the observations in the latent space. VAE and its flavours are one of the first and most popular models for unsupervised anomaly detection~\citep{an2015variational,xu2018unsupervised} Unlike an autoencoder, the encoder of the VAE describes the probability distribution of each latent attribute. During training, the model computes a latent space representation (LSR) of the non-anomalous input image. The latent space in VAEs is continuous by design and allows easy random sampling and interpolation. This is achieved by designing the encoder to output two vectors:  a vector of means $\mu$ of data samples and a vector of standard deviations $\sigma$. The encoding is generated within these distributions. The decoder learns that not just a single point but all the points around it are referred to as a sample of the same class, thus decoding even slight variations of the encoding. Typically, the network is trained by optimising the evidence lower bound (ELBO) $L$, which can be defined as:

\begin{equation}
\log p(x) \geq L=-D_{K L}(q(z \mid x) \| p(z))+E_{q(z \mid x)}[\log p(x \mid z)]
\end{equation}
where, q(z$\mid$ x) and  p(x$\mid$ z) are diagonal normal distributions that are parameterised by neural networks $f_\mu$, $f_\sigma$, and $g_\mu$, and constant $c$ such that:

\begin{equation}
\mathrm{q}(\mathrm{z} \mid x)=N\left(z ; f_{\mu, \theta 1}(x), f_{\sigma, \theta 2}(x)^{2}\right)
\end{equation}
\begin{equation}
p(x \mid z)=N\left(x ; g_{\mu, \gamma}(z), I * c\right)
\end{equation}
 
\subsection{Vector  Quantized  Variational  autoencoder}
\label{sec:VQVAE}
Vector Quantised-Variational AutoEncoder (VQ-VAE) \citep{oord2017neural,marimont2020anomaly} framework encodes the images in categorical latent space. Further, an auto-regressive (AR) model is used to model the prior distribution of latent codes. The prior probability approximated by the AR model is then used for unsupervised anomaly detection and gives the sample and pixel-wise anomaly scores. The encoder of the VQ-VAE framework is based on a dictionary mapping K discrete keys into a D-dimensional embedding space, i.e., observed variables are mapped to the embedding space, $z_e(x) \in R^D$. The posterior in VQ-VAE is defined as :
\begin{equation}
    q(z = k \mid x) = 
    \begin{cases}
            1, & for k = \operatorname*{arg\,min}_j || z_e(x) - e_j ||_2\\
    0, & \text{otherwise}
    \end{cases}
\end{equation}
The embedding in the dictionary nearest to the encoder's output is given to the decoder as an input, i.e.,$z_q(x) \sim q(z\mid x)$. The decoder then reconstructs the distribution $p(x\mid z_q(x))$.The VQ-VAE Loss function is therefore defined as:
\begin{equation}
  L = log(x\mid z_q(x)) + \mid\mid sg[z_e(x)]-e\mid\mid_2^2 + \mid\mid sg[e] - z_e(x)\mid\mid_2^2  
\end{equation}
where $sg[.]$ is the stop gradient operator.
Further, an AR model is employed to learn the prior distribution of VQ-VAE, and the probability of samples is approximated. The samples with low probability are identified as anomalies. AR models generate multiple restorations as they are generative models and allow sampling of one variable at a time in an iterative manner. 

\subsection{Gaussian  Mixture  Variational  Autoencoder}
\label{sec:GMVAE}
The Gaussian  mixture  variational  autoencoder \citep{dilokthanakul2016deep,chen2020unsupervised}  approach (GMVAE) combines image restoration techniques with unsupervised learning - used in various anomaly detection approaches~\citep{guo2018multidimensional,fan2020video}. A GMVAE is first trained on an anomaly-free dataset to learn a normative prior distribution. A Maximum-A-Posteriori (MAP) restoration model then uses this prior to detecting the outliers. In GMVAE, the ELBO is formally expressed as:
    \begin{equation}
    \begin{aligned}
     \mathbb{E}{q(z\mid X)} [log p(X\mid z)] - \mathbb{E}{q(\omega \mid X) p(c \mid z, \omega)} \\
             [KL [q(z \mid X) | p(z \mid \omega, c)]]\\
             - [KL [q(\omega \mid X) | p(\omega)]] - \mathbb{E}_{q(z \mid X) q(\omega \mid X)} \\
             [KL [p(c \mid z, \omega) | p(c)]]
    \end{aligned}
    \end{equation}
            
where the first part is the reconstruction term, the second part ensures the encoder distribution fits the prior, the third term does not let the posterior $\omega$ diverge from the prior $p(\omega)$, and the last term enforces the model to not collapse into a single Gaussian but uses the mixture model. For the architectural choice, seven convolutional layers for the encoder and seven transpose layers for the decoder are used. The latent variables $z$ and $\omega$ are 2D structures with size (32, 42 1) and nine clusters, c.

\subsection{Context-encoding Variational Autoencoder}
\label{sec:ceVAE}
The core idea of Context-encoding Variational Autoencoder (ceVAE) \citep{zimmerer2018context} is to combine the reconstruction term with a density-based anomaly scoring. This allows using the model-internal latent representation deviations and an expressive reconstruction term on the samples and individual pixels. The overall architecture comprises of fully convolutional encoders $f_u$, $f_\sigma$ and a decoder unit $g$, where the context encoding part used the encoder module for a data sample. ceVAE can be divided into two branches: VAE branch and CE branch.

\paragraph{\textbf{VAE Branch}:} The deviations of the latent from the CE branch is further inspected. The encoders $f_u, f_\sigma$, the decoder g, and a standard diagonal Gaussian prior p(z) are used in the VAE module with an objective function:
    
    \begin{equation}
    L_{VAE} = L_{KL} (f_\mu(x), f_\sigma(x)^2) + L_{recVAE}(x, g(z))
    \end{equation} 
    
    where $z \sim \mathcal{N}(f_\mu(x), f\sigma(x)^2)$ with the reparameterisation trick and $L_{KL}$ loss with a standard Gaussian yield a comparable anomaly score. KL-loss is used to analyse the deviations of posterior from the prior. 
    
    \paragraph{\textbf{CE branch}:} sample $x$ is subjected to context encoding noise by masking specific regions. Training occurs by reconstructing the perturbed input $\hat{x}$ using the encoder $f_\mu$ and the decoder g, formally, $L_{rec CE}(x, g(f_\mu(\hat{x})))$. The results show CEs are more discriminative and semantically produce rich representations, which positively influences the expressiveness of model variations. 
    
    \paragraph{\textbf{ceVAE}:} On combining the above modules, the aim is to capture both the effects, i.e., a better-calibrated reconstruction loss and model-internal variations. The objective function is restructured as the following: 
    
    \begin{equation}
    \begin{aligned}
    L_{ceVAE} = L_{KL}(f_\mu(x), f_\sigma(x)^2) \\ 
                + L_{recVAE}(x, g(z)) + L_{recCE}(x, g(f_\mu(\hat{x})))
    \end{aligned}
    \end{equation}
    
    where $L_{KL}$ is the KL-loss, z is sampled with the reparameterisation method, and $\hat{x}$ is perturbed by masking regions similar to CEs. During the training process $L_{recCE}$ has no constraints for normality on the prior $p(z\mid x)$. The combination of CE and VAE has a regularising effect that prevents the posterior from collapsing and better represents the semantics in the input data.

    % \begin{figure*}[h!]
    %     \centering
    %     \includegraphics[width=0.9\textwidth] {figs/cevae.png}
    %     \caption{ceVAE model architecture.} 
    %     \label{fig: cevae}
    % \end{figure*}

\subsection{Hypothesis behind StRegA}
Even though VAEs have their advantages, like they can can be less computationally expensive than transformers, but have been seen to struggle to detect anomalies in clinical data. The reason for this could be the differences between the training and testing sets in terms of image properties (e.g. contrast). One possible way to improve their performance would be to "simplify" the input to the model - making it easier for the model to learn a distribution of the anomaly-free data - which might also help the model generalise better. Hence, this paper focuses on developing a VAE-based technique focusing on output "simplification" to improve the model's performance on clinical data.

==> sections/2_methodology.tex <==

\section{Methodology}
\label{sec:methods}

\subsection{Study of existing methods and baseline selection}
Autoencoders and their flavours are commonly used for unsupervised anomaly detection as discussed in~\ref{sec:relatedwork}. While selecting the baselines, the aforementioned methods were compared and finally, the best performing baseline (i.e. ceVAE) was selected and modified to develop the proposed approach.
\subsection{StRegA : Segmentation Regularised Anomaly }
The proposed unsupervised anomaly detection pipeline, StRegA: Segmentation Regularised Anomaly - shown in Fig.\ref{fig:StRegA}, includes a modified compact version of the Context-encoding Variational Autoencoder (ceVAE) \citep{zimmerer2018context} - Compact ceVAE (cceVAE), combined with pre and postprocessing steps. Anomaly detection is performed in 2D, per-slice basis. The input volumes are preprocessed in 3D, then slices are supplied to the model, followed by that, postprocessing steps are applied, and finally, the slices are stacked together to obtain the final result in 3D. It is worth mentioning by splitting the 3D volumes into 2D slices, the spatial context within the volumes is lost. But this was done to make the training process feasible in terms of GPU requirements. The code of StRegA is publicly available on GitHub~\footnote{StRegA on GitHub: \url{https://github.com/soumickmj/StRegA}}.

\begin{figure*}%[h!]
    \centering
    \includegraphics[width=0.95\textwidth] {figs/strega.png}
    \caption{StRegA pipeline} 
    \label{fig:StRegA}
\end{figure*}

\subsubsection{Preprocessing}
\label{sec:Preprocessing}
The first preprocessing step was to segment the input image into different tissue types and obtain the corresponding segmentation mask. Segmentation means partitioning the input images into various segments. Segmentation can simplify the input given to the model as the model needs to deal with less variations in the input images that can help improve the performance of the anomaly detection system. Segmentation helps standardise the input images with different image properties, such as images with different MR contrasts (e.g. T1w, T2w). This was performed by supplying the 3D brain images to the automatic segmentation tool of FSL (\cite{jenkinson2012fsl}) - FAST, which segmented the brain into three different tissue types: grey matter, white matter, cerebrospinal fluid (CSF); and background - a total of four classes. The segmentation command of FSL FAST has a flag to select the modality of the input volume (e.g. T1w, T2w). Rest of the parameters of FSL FAST (apart from the number of classes and the type of the image) were kept to their default values. The underlying principle of FAST is formulated on a hidden Markov random field model and an associated expectation-maximisation algorithm. The entire process is automated and is capable of producing a probabilistic/partial volume tissue segmentation. Apart from segmenting the input volume, this tool also corrects spatial intensity variations (also known as bias field or RF inhomogeneities). The segmentation mask was normalised with the intensity distribution of the dataset - normalised with zero mean and unit variance. The volumes were divided into 2D slices in the axial orientation, and then they were resized to 256×256 in-plane using bilinear interpolation before feeding them into the network. During the training phase, in addition to the above-mentioned preprocessing steps, data augmentation was also performed. The augmentation techniques used can be split into two groups: intensity-based and spatial augmentation. Intensity augmentation included bias field artefacts, Gaussian noise,  random gamma, and ghosting artefacts. While spatial augmentation consisted of horizontal flipping, vertical flipping, affine transformations, and rotation with a degree between -15 and +15.

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=0.45\textwidth] %{figs/preprocess.png}
%    \caption{FSL FAST Segmentation}
%    \label{fig:preprocess}
%\end{figure}


%\begin{figure*}
%    \centering
%    \includegraphics[width=0.9\textwidth] %{figs/Preprocess_BD.png}
%    \caption{Pre-processing}
%    \label{fig:Preprocess_BD}
%\end{figure*}

\subsubsection{Network Model: cceVAE}
\label{sec:model}



This work proposes a compact modified version of the ceVAE model \citep{zimmerer2018context}, explained in Sec.\ref{sec:ceVAE}: Compact ceVAE(ccVAE). A representational diagram of the network has been shown in Fig.~\ref{fig:cceVAE}. This is a compact version as it has smaller encoder and decoder than the original ceVAE - having a symmetric encoder-decoder with 64, 128 and 256 feature maps and a latent variable size of 256. The authors hypothesise that a more compact version of the network will reduce any possibilities of overfitting, especially for data that is more simplified than un-processed slices - where many learnable parameters might not be required. This proposed model also uses residual connections and batch normalisation layers - which were not present in ceVAE. The preprocessed images are fed into this network model, and the network tries to reconstruct the input. During training, anomaly-free (in the experiments of this paper: healthy brain MRIs) images are provided, and the network attempts to learn a Gaussian distribution of the given anomaly-free dataset. While inference, the network attempts to reconstruct the input image from the learnt Gaussian distribution. If the network encounters images with anomalies - they are then out-of-distribution samples. Hence, the network should "in-theory" fail to reconstruct the anomalies as they do not belong to the learnt distribution. The reconstruction difference is then computed by subtracting the model's output from its input to generate the initial anomaly mask - which is then postprocessed to finally detect the anomaly.

\begin{figure*}%[h!]
    \centering
    \includegraphics[width=0.95\textwidth] {figs/c_cevae.png}
    \caption{The proposed Compact ceVAE architecture: cceVAE. Each of the convolution blocks contains a convolution layer with the mentioned configuration, followed by a batch normalisation layer.} 
    \label{fig:cceVAE}
\end{figure*}

\subsubsection{Postprocessing}
\label{sec:Postprocessing}
After subtracting the reconstruction from the model's input, the initial anomaly mask is obtained - containing values between zero and one, where one implies anomaly while zero means no anomaly. Then this mask is first thresholded to eliminate any pixel having a value less than zero by replacing all the negative values with zero. Then to remove the intensity outliers, the mask was thresholded using Otsu's method \footnote{\url{https://en.wikipedia.org/wiki/Otsu's_method}}. The Otsu thresholding was applied individually on each output slice - resulting in different suitable thresholds for each slice of each subject. Otsu is a frequently used method for performing automatic image thresholding, which divides all the pixels into two classes - background and foreground, based on a single intensity threshold. The threshold is calculated by minimising intra-class intensity variance, or in other words, by maximising inter-class variance. \footnote{\url{http://www.labbookpages.co.uk/software/imgProc/otsuThreshold.html}}. 

This results in a binary anomaly mask. After performing Otsu thresholding, the small irrelevant parts of the mask are removed by applying morphological opening \footnote{\url{https://en.wikipedia.org/wiki/Opening_(morphology)}} - which removes all bright structures of an image with a surface smaller than the area threshold. It is equivalent to applying dilation on top of erosion on the image. This gives the final anomaly mask. It is then resized through interpolation to whichever input size the original image had before resizing during preprocessing. Finally, all the slice-wise 2D masks are stacked together to get the final anomaly mask in 3D.

%\begin{figure*}[h!]
%    \centering
%    \includegraphics[width=0.9\textwidth] %{figs/postprocess_BD.png}
%    \caption{Post-processing} 
%    \label{fig:postprocess_BD}
%\end{figure*}


\subsection{Datasets}
\label{sec:Datasets}
Training unsupervised anomaly detection models warrant anomaly-free datasets. As the focus of this paper is on brain MRIs, two anomaly-free datasets were selected for training the models: MOOD challenge dataset \citep{mood_2021_4573948} and IXI dataset \footnote{IXI Dataset: \url{ https://brain-development.org/ixi-dataset/}}. It is worth mentioning that even though both the datasets contain MRIs only from normal, healthy subjects - there might still be some anomalies present in some of the MRIs that the experts missed. However, in this research, following the authors of the datasets - these datasets were considered to be comprised of only anomaly-free healthy brain MRIs. MOOD dataset comprises 800 T1w brain MRIs with a matrix size of 256x256x256 - 700 of which were used for training, and 100 were held out for testing, while the IXI dataset contains MRIs of nearly 600 subjects - all of which were used in training, acquired using 1.5T and 3T MRIs in three different hospitals, with different MRI sequences: T1w, T2w, PDw, MRA, and DTI. In this research, T1w and T2w images from the IXI dataset were used separately - for training separate T1 and T2 models. Trainings were performed by combining MOOD with one of the IXI contrast: MOOD+IXIT1 and MOOD+IXIT2. Due to the fact that the models worked with segmented volumes (see Sec.~\ref{sec:Preprocessing}, it was possible to combine MRIs with different contrasts in the training set as the segmentation helps to standardise them. However, the segmentation still has some minute differences in the different contrasts, especially in terms of the tumour delineation. Hence, the motivation behind combining different datasets (and contrasts) was to make the model more robust against inter-dataset variations (e.g. resolution), including differences in contrasts in the test set than in the training set.

For evaluating the approach with a dataset with clinical anomalies, 80 randomly selected volumes from BraTS 2017 \footnote{BraTs: \url{https://www.med.upenn.edu/sbia/brats2017/data.html}} dataset was used, which contains four types of MRIs with high and low-grade brain tumours: T1-weighted, and contrast-enhanced T1-weighted (with contrast agent), T2-FLAIR, and T2-weighted. This paper used contrast-enhanced T1-weighted (T1ce) and T2-weighted MRIs. Additionally, the model was also tested on the "toy test set" provided in the MOOD dataset, comprising one anomaly-free and three anomalous MRIs containing artificial anomalies. It is noteworthy that the image contrasts, acquisition parameters, and other image properties of the BraTS dataset are very different from the training sets. Hence, a controlled synthetic anomalous dataset was created as a part of this research - to evaluate the approach on a dataset that contains anomalies, but the contrast and other image characteristics are similar to the training set. 

\subsubsection{Generating Synthetic Anomalous Dataset}
\label{sec:Synthetic_Datasets}
\begin{figure}%[h!]
    \centering
    \includegraphics[width=0.48\textwidth] {figs/MOOD_brats.png}
    \caption{Synthetic MOOD image generated using anomaly from BRATS data set, including one anomaly-free example in the last row}
    \label{fig: syn}
\end{figure}
An artificial controlled test set was created by superimposing anomalies from the BraTS dataset onto the held-out test-set containing anomaly-free brain MRIs. This was performed to evaluate the performance of the methods when the non-anomalous parts of the images have similar contrast and other characteristics as the training dataset - to solely evaluate the performance of the model when the model doesn't encounter any other difficulties, while it also ensures that the artificial "tumours" are realistic.  

To generate the synthetic anomalous dataset, the anomalies (i.e. tumours) from 20 volumes of the BRATS dataset were extracted by multiplying the ground truth tumour masks with the brain images. Then the intensity values of the tumours were normalised between 0 and 1, and the resultant outputs were interpolated as 256x256 slices. These 20 extracted tumours were superimposed onto 20 randomly-selected volumes from the anomaly-free held-out test-set from the MOOD dataset, which places the tumours on top of the anomaly-free brain images. This creates a set of synthetic anomalous test data which can be used in conjunction to test the performance of the pipeline. Consider a BraTS image sample B, and its corresponding ground-truth segmentation mask S from the dataset pointing out the tumour, then the superimposed MOOD image (from the held-out test-set) sample A of corresponding slice from h slices can be calculated as :

\begin{equation}
  \begin{array}{l}
    A'_{i} = A_{i} + M_{i}\ ; \forall i \in h \text{ ,where }    \\ \cr
     M_{j} = B_{j}\ .\ S_{j}\ ; \forall j \in h
  \end{array}
\end{equation}

% Figure \ref{fig: syn} shows various IXI datasets with synthetically generated anomalies. 



==> sections/3_evaluation.tex <==
\section{Experiments and Evaluations}
\label{sec:results}
The methods were compared based on their accuracy in segmenting the anomalies, calculated with Sørensen–Dice coefficient. Initial experiments were performed using a vanilla VAE~\citep{mickISMRM21Anomaly}, following that, different state-of-the-art models (the ones mentioned in Sec.~\ref{sec:relatedwork}) were compared. Finally, the three best-performing models in this current experimental setup were chosen as baselines, and final comparisons were performed against the proposed method.

\subsection{Initial Selection of Baseline Models}
The initial approach of using the vanilla VAE~\citep{mickISMRM21Anomaly} was able to detect simple contrast anomalies - anomalies having very different contrast than the rest (e.g. MOOD toy dataset), but in most cases failed to generate an acceptable reconstruction. SkipAE~\citep{cccc} resulted in better detection of anomalies. While the results on the synthetic data and the MOOD toy test data were better, the more complicated anomalies were harder to detect in the reconstructions. Other models, which are explained in Sec.~\ref{sec:relatedwork} were also experimented with, and it was found that the ceVAE~\citep{zimmerer2018context}~(Sec.~\ref{sec:ceVAE}) performed the best when it comes to segmenting pathological anomalies. Hence, this was chosen as the primary baseline of this paper. The second and third best performing models, GMVAE~\citep{chen2020unsupervised}~(Sec.~\ref{sec:GMVAE}) and SkipAE~\citep{cccc}~(Sec.~\ref{sec:SkipAE}) respectively, were also chosen as additional baselines. 

\subsection{Method Development}
\label{sec:method_Dev}
This research focused on simplifying the input to the backbone model - by introducing different preprocessing techniques. It was observed that using segmentation as a preprocessing step assisted the models most and improved the model's performance which was tested with all the baseline models. Fig.~\ref{fig:fastseg} shows a few examples of T1w and T2w slices with tumours applying FSL FAST - to visualise how this preprocessing segmentation performs while working with the BraTS dataset that contains tumours. It was observed that the tumour was usually made part of the CSF class, however, lacks proper delineation. Apart from the tumour, the actual CSF is also part of this class - making it impossible to use these as final tumour segmentations. When this particular class was compared against the corresponding tumour masks, the resultant Dice scores were 0.196±0.116 and 0.202±0.137 for T1w and T2w volumes from the BraTS dataset. Hence, it is required to further proceed with the anomaly detection pipeline to finally localise and segment the tumour. Moreover, as stated earlier, the segmentation step helps to make the MRIs of different contrasts similar - that can also be observed in Fig.~\ref{fig:fastT1}~and~\ref{fig:fastT2}.

\begin{figure}%[h!]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth] {figs/t1_seg_color.png}
         \caption{T1w}
         \label{fig:fastT1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth] {figs/t2_seg_color.png}
         \caption{T2w}
         \label{fig:fastT2}
     \end{subfigure}
    
    \caption{Examples of segmented T1w and T2w volumes using FSL FAST}
    \label{fig:fastseg}
\end{figure}




Different other preprocessing techniques were also experimented with, and the final set of techniques was made part of the StRegA pipeline - explained in Sec.~\ref{sec:Preprocessing}. When experimenting with the number of layers in the encoder and decoder of the ceVAE model with these preprocessing techniques, it was observed that the results on the test datasets improved significantly when a more compact model was used. This could be due to the fact that a more compact model reduces the risk of over-fitting on the relatively simpler segmented data. Thus after several experiments, having symmetric 64, 128 and 256 feature maps and a latent variable size of 256 yielded the best generalisation in reconstruction quality. Implementing skip connections as was used in SkipAE provided no meaningful improvements, but residual connections with batch normalisation provided better results and were thus included in the model - results in the final cceVAE model~(Sec.~\ref{sec:model}).%
For the experiments here, the proposed model was trained with the Adam optimiser~\citep{kingma2014adam} using a learning rate of 1e-4 and a batch size of 64 for 70 epochs.


\subsubsection{Comparative Results}

The proposed StRegA pipeline was compared against the three baseline models and an additional baseline - by combining the StRegA preprocessing steps with the ceVAE model. Fig.~\ref{fig:compare_res} shows a qualitative comparison of the different methods. It can be observed that the proposed StRegA pipeline provides a more localised detection of the anomaly compared to the other methods. Tables~\ref{tab:t1comparenumbers}~and~\ref{tab:t2comparenumbers} portray a quantitative comparison of the T1 and T2 models. The proposed method outperformed all the other models with statistical significance in both T1 and T2 cases while achieving 49\% and 82\% improvements in Dice scores over the baseline ceVAE for the task of segmenting tumours from T1w and T2w brain MRIs from the BraTS dataset, resulting in average Dice scores of 0.531±0.112 and 0.642±0.101, respectively. A separate model was also trained only on the IXI T2w dataset and was then tested using the BraTS T2w dataset, resulting in an average Dice score of 0.631±0.117 which is 1.7\% less than the model trained on a combination of MOOD (T1) and IXI T2. This can bee attributed to the fact that this specific training had a smaller training set than the combined one. Another additional evaluation was performed by applying the MOOD-IXIT2 traine StRegA on the BraTS T1 images, and it resulted in an average Dice score of 0.533±0.179 (similar to BraTS T1 results on the model trained on MOOD-IXTT1, only 0.38\% better). This not only shows that having more data is better but also the limits of the model on BraTS T1.



It can be observed that all the models perform better in the case of T2 than on T1ce. This can also be either because the tumours are easier to detect in T2 images than on T1ce images and could also be because of the segmentation performance of FSL in case of anomalous data, as FSL is typically used for anomaly-free images. Moreover, Fig.~\ref{fig:violin_compare_res} compares the range of resulting Dice scores for the task of anomaly detection in BraTS T2 images for ceVAE, ceVAE with StRegA preprocessing, and StRegA, with the help of violin plots. The white dot inside each of the violins represents the median Dice score, the thick black bar at the centre exhibits the interquartile range, and the thin dark line depicts the rest of the distribution excluding outliers. It can be seen that the segmentation assists the ceVAE model in achieving better scores, while the complete StRegA pipeline manages to improve the scores even further. StRegA results in a higher overall median Dice score than both the other methods, while its worst outlier is still better than the worst outliers of the other methods. Finally, Figures~\ref{fig:t1-final}~and~\ref{fig:t2-final} show the output of the different stages of the pipeline for BraTS T1 and T2, respectively. Similarly, Fig.~\ref{fig:syn-final} shows the stages for synthetic anomalies. 

\begin{figure}%[h!]
        \centering
        \includegraphics [width=0.49\textwidth] {figs/violin.png}
        \caption{Violin plot comparing predictions on BraTS T2 data} 
        \label{fig:violin_compare_res}
\end{figure}




% ----

% ----
% ----
\subsubsection{StRegA as an Assistive Technology}
The earlier comparisons have demonstrated the proposed pipeline's superiority over the baseline models. However, several cases of under-segmentation were observed. Detecting if there is any anomaly or providing the location of the anomaly might also be sufficient to improve the clinical workflow by assisting the radiologists in filtering anomalous cases and getting an approximate location of the same. Figures.~\ref{fig:anomaly_locallise_T1}~and~\ref{fig:anomaly_locallise_T2} show the potential of using StRegA as an assistive technology to localise the anomalies in the MRIs for BraTS T1ce and T2, respectively. This was achieved by creating bounding boxes around the prediction of StRegA, and they were compared against the bounding boxes generated from the ground-truth labels. It can be observed that the proposed method was able to properly locate the anomalies. As seen earlier, the T2 results were better than the T1ce ones. For T1ce, under-estimations were observed most of the time. However, for T2, the results are better, and most of the time, StRegA managed to mark them appropriately. Despite the under-estimations, the results show the potential of using this method as assistive technology - as a decision support system.     


\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth] {figs/t1_bbox_new.png}
    \caption{Anomaly localisation : BraTS T1ce}
    \label{fig:anomaly_locallise_T1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth] {figs/t2_bbox_new.png}
    \caption{Anomaly localisation : BraTS T2}
    \label{fig:anomaly_locallise_T2}
\end{figure}
%\begin{figure}%[h!]
%        \centering
%        \includegraphics [width=0.45\textwidth] {figs/t1_bbox.png}
%        \caption{Anomaly localisation : BraTS T1ce} 
%        \label{fig:anomaly_locallise_T1}
%\end{figure}

%\begin{figure}%[h!]
%        \centering
%        \includegraphics [width=0.45\textwidth] {figs/t2_bbox.png}
%        \caption{Anomaly localisation : BraTS T2} 
%        \label{fig:anomaly_locallise_T2}
%\end{figure}





==> sections/4_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
The results demonstrate that the proposed StRegA pipeline achieved significantly better scores than the baseline models in detecting brain tumours and artificial anomalies while being trained on anomaly-free brain MRIs. The proposed pipeline aims at simplifying the input to the model by segmenting it. This same step also helps the model to generalise better in terms of the changes in contrast - which can be seen from the results of the models on the BraTS dataset. MOOD toy and the synthetic anomalous datasets had the same image contrast and resolution as the training dataset - on which the baseline models achieved comparable results, while BraTS had considerably different contrast - on which the baseline models struggled the most. Due to the fact that the input is simpler, a less-complex model has been seen to be sufficient (i.e. cceVAE instead of ceVAE). This helps in reducing the memory requirement - making it possible to work with more commonly-available hardware, and also reduces the chances of overfitting as the model has less number of trainable parameters.

Even though StRegA has performed significantly better than the baseline models, it is to be noted that the predictions are not perfect - which is commonly seen with UAD techniques, and there is a strong dependency on the preprocessing steps, as can be seen from the results of ceVAE and ceVAE with StrRegA preprocessing. It is also worth mentioning as FSL segmentation is typically used on anomaly-free images, using them on anomalous data might have induced some bias in the training-testing of the models which is not possible to quantify. Moreover, it was observed that the compact version of ceVAE proposed here performed better than the original ceVAE model, which might be attributed to the fact that the preprocessed images require a much simpler representation than images without preprocessing - consequently requiring less number of trainable parameters to learn the distribution of healthy-brain. Another interesting observation can that can be made from the results is that the models performed 21\% better on T2w images than T1ce from the BraTS dataset, even while being trained to focus on T1w images (T1ce was tested on models trained on purely T1w images, T2s were tested on models trained on a combination of T1 and T2). This can be because the tumours are easier to distinguish in T2 than in T1ce due to the significant intensity difference between tumour and non-tumour tissues. It can also be due to some bias induced by the FSL's segmentation. 

Undersegmentations can be observed in all the examples. This also resulted in a complete disappearance of a small anomaly as can be seen in Fig.~\ref{fig:t1-final}~(row 2). Hence, one immediate point of concern is the size of the anomaly in the input image. As morphological opening would eliminate the prediction if it is too small, the StRegA postprocessing steps might not be ideal for detecting small anomalies, e.g. multiple sclerosis. One way to deal with the small anomalies would be to reduce the area threshold. For synthetically generated anomalies, the pipeline performed almost perfectly, as can be seen in Fig.~\ref{fig:syn-final}. Nevertheless, these models were trained in an unsupervised fashion – without any labelled training data. Hence, the requirement of large manually annotated training data can be mitigated. The anomalies detected by such a method can also be further used as weak labels to train weakly-supervised or semi-supervised models - which might improve the final segmentation quality without requiring much manual intervention.   

StRegA, similar to the baselines experimented here, works in 2D and relay upon the model's reconstruction error. This way of detecting anomalies is suitable for local structural anomalies, such as tumours, but might not be suitable for detecting changes in brain atrophy, such as the change in brain atrophy due to the Alzheimer's disease. Going for a 3D method and extending the way of detecting the anomalies might help the method detect such anomalies.

StRegA as an assistive technology might help radiologists notice anomalies that might otherwise be overlooked. Diagnostics by radiologists remain undiscovered in up to 5-10 \% of cases \citet{bruno2015understanding}. The cause of these errors is due to unintentional bias, where radiologists focus more on the centre part of the MRI while neglecting peripheral findings. The ever-increasing number of radiological images for assessment increases the workload in radiology which in turn can result in more missed brain pathologies. The presented method might assist in localising anomalies (as seen in Fig.~\ref{fig:anomaly_locallise_T2}~and~\ref{fig:anomaly_locallise_T2}) and improve the overall diagnostic accuracy. %\newpage

==> sections/5_conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}
This paper address the challenge of anomaly detection in an unsupervised manner by presenting an unsupervised anomaly detection system named StRegA: \textbf{S}egmen\textbf{t}ation \textbf{Reg}ularised \textbf{A}nomaly, which combines a modified and compact version of the ceVAE model (cceVAE) with pre- and postprocessing steps. The proposed method was trained using anomaly-free brain MRIs from two benchmark datasets and was then evaluated for the task of detection of brain tumours. The proposed method was compared against four baselines and outperformed all of them with statistical significance. StRegA achieved Dice scores of 0.531±0.112 and 0.642±0.101 while segmenting tumours, as well as 0.723±0.134 and 0.859±0.112 while segmenting artificial anomalies, from T1w and T2w MRIs, respectively - resulting in 49\%, 83\%, 5\%, and 21\% improvements, respectively in the four scenarios, over the best performing baseline model ceVAE, while achieving 2\%, 23\%, 2\%, and 10\% improvements over ceVAE with StRegA preprocessing. Undersegmentations were observed in most cases, however, the method could localise the anomalies properly. This work has shown the potential of using this method as part of a decision support system. 

In the future, this method will be evaluated for the tasks of detecting other types of anomalies than brain tumours - to evaluate its generalisability to other pathologies. 
The current method faces difficulties while detecting small anomalies - this might be addressed by modifying the postprocessing steps. Furthermore, techniques other than segmentation to simplify the input to the model will also be evaluated in the near future.



==> sections/n_bigfigs.tex <==


\begin{table*}%[h!]
  \begin{center}
    \caption{Comparative results of StRegA with other models on T1 data.}
    \label{tab:t1comparenumbers}
    \begin{tabular}{ |c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\bfseries Model} & 
    \multicolumn{3}{|c|}{\bfseries Dice Score ($\mu\pm\sigma$)} \\
    \cline{2-4} 
     & MOOD Toy Data & Synthetic Anomalous Data &  BraTS T1w \\
    \hline
    SkipAE & 0.443 $\pm$ 0.136 & 0.498 $\pm$ 0.164 & 0.209 $\pm$ 0.113\\
    \hline
    GMVAE & 0.657 $\pm$ 0.121 & 0.711 $\pm$ 0.105 & 0.337 $\pm$ 0.124\\
    \hline
     ceVAE & 0.633 $\pm$ 0.145 & 0.690 $\pm$ 0.164 & 0.356 $\pm$ 0.132\\
    \hline
     ceVAE (with StRegA preprocessing) & 0.724 $\pm$ 0.132 & 0.710 $\pm$ 0.111 & 0.520 $\pm$ 0.108\\
    \hline
    \textbf{StRegA}  & 0.737 $\pm$ 0.098 & 0.723 $\pm$ 0.134 & 0.531 $\pm$ 0.112\\
    \hline
    \end{tabular}
  \end{center}
\end{table*}
% ----
\begin{table*}%[h!]
  \begin{center}
    \caption{Comparative results of StRegA with other models on T2w data.}
    \label{tab:t2comparenumbers}
    \begin{tabular}{ |c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\bfseries Model} & 
    \multicolumn{3}{|c|}{\bfseries Dice Score ($\mu\pm\sigma$)} \\
    \cline{2-4} 
     & MOOD Toy Data & Synthetic Anomalous Data &  BraTS T2 \\
    \hline
    SkipAE & 0.517 $\pm$ 0.145 & 0.498 $\pm$ 0.173 & 0.221 $\pm$ 0.101\\
    \hline
    GMVAE & 0.699 $\pm$ 0.121 & 0.701 $\pm$ 0.121 & 0.340 $\pm$ 0.167\\
    \hline
     ceVAE & 0.724 $\pm$ 0.145 & 0.712 $\pm$ 0.132 & 0.350 $\pm$ 0.071\\
    \hline
     ceVAE (with StRegA preprocessing) & 0.797 $\pm$ 0.099 & 0.783 $\pm$ 0.111 & 0.522 $\pm$ 0.135\\
    \hline
    \textbf{StRegA}  & 0.856 $\pm$ 0.098 & 0.859 $\pm$ 0.112 & 0.642 $\pm$ 0.101\\
    \hline
    \end{tabular}
  \end{center}
\end{table*}
% ----


% ----
\begin{figure*}%[h!]
        \centering
        \includegraphics [width=0.9\textwidth] {figs/compare_analysis.png}
        \caption{Comparative results from different methods. Top row: artificially generated anomalous data. Bottom row: BraTS T2w image. (a) A slice from the input volume, (b) ceVAE, (c) SkipVAE, (d) GMVAE, (e) StRegA and (f) ground truth} 
        \label{fig:compare_res}
\end{figure*}
% ----

\begin{figure*}%[h!]
        \centering
        \includegraphics [width=0.8\textwidth] {figs/syn_pipeline.png}
        \caption{StRegA results on synthetically generated data} 
        \label{fig:syn-final}
\end{figure*}
% ----

% ----
\begin{figure*}%[h!]
        \centering
        \includegraphics [width=\textwidth] {figs/t1-final.png}
        \caption{StRegA results on BraTS dataset (T1) images (a) Input Image (b) Segmented Image (c) Reconstruction (d) Manual and Otsu thresholding (e) Morphological Opening -> \textbf{Final prediction} (f) Ground Truth} 
        \label{fig:t1-final}
\end{figure*}
% ----
\begin{figure*}%[h!]
        \centering
        \includegraphics [width=\textwidth] {figs/t2-final.png}
        \caption{StRegA results on BraTS dataset (T2) images (a) Input Image (b) Segmented Image (c) Reconstruction (d) Manual and Otsu thresholding (e) Morphological Opening \textbf{Final prediction} (f) Ground Truth} 
        \label{fig:t2-final}
\end{figure*}
% ----

==> sections/x_extra_data.tex <==
\section{Data}
\label{ch:data}

\subsection{Data sets}
\label{sec:Data sets }

Brain tumor segmentation (BraTS) 2019 \footnote{BraTs: \url{https://www.med.upenn.edu/sbia/brats2017/data.html} (Date acc: September,20,2020)}, Medical Out-of-Distribution Analysis Challenge (MOOD) dataset \footnote{MOOD: \url{https://zenodo.org/record/3961376} (Date acc: October,10,2020)}, and IXI dataset \footnote{IXI Dataset: \url{ https://brain-development.org/ixi-dataset/} (Date acc: November,05,2020)} were used in this experiment. All three datasets are three-dimensional whole-brain MR images, while the BRaTs dataset contains pixel-wise anomaly annotations. The other two data sets, namely IXI and MOOD, are samples from normal, healthy subjects. The healthy subject images and anomalous subject images are classified with the use of provided annotation.

IXI dataset contains nearly 600 MR images from normal healthy subjects and consists of t1, t2, and PD weight images.  MOOD dataset consists of 500 scans of brain MRI of dimensions 256 * 256 * 256, which are hand-selected scans with no anomalies.  BraTS is a dataset for glioblastoma and lower grade glioma and has the four contrast images of T2 FLAIR, T2-weighted, T1-weighted, and T1-weighted with contrast agent. 

The process of training and testing included different datasets. The proposed models were trained on the MOOD+IXI dataset and tested on the BRaTs dataset. Additionally, the model was evaluated on IXI and MOOD toy dataset, which was created synthetically. Artificial anomalies were imposed on these healthy datasets to test the model boundaries. Evaluating the validation data can provide the results regarding abnormal tissues and normal tissues since anomaly images invalidation data usually contain both normal and abnormal tissues. 

\subsection{Preprocessing}
\label{sec:Preprocessing}

The training dataset consisted of images from IXI and MOOD datasets. The healthy images were preprocessed with several approaches before passing them as the model inputs. The first preprocessing step included. The first step included skull stripping and co-registration between multi-contrast images. This was followed by segmentation of the 3D brain image using  FAST FSL \footnote{FSL: \url{https://fsl.fmrib.ox.ac.uk/fsl/fslwiki/FAST} (Date acc: March,10,2021}.  FMRIB's Automated Segmentation Tool (FSL) segments a 3D image of the brain into different tissue types (Grey Matter, White Matter, CSF, etc.) while also correcting for spatial intensity variations (also known as bias field or RF inhomogeneities). The segmented image was normalized and standardized with the intensity distribution of the dataset normalized with zero mean and unit variance. 
All images were resized to 256× 256 by using bilinear interpolation. Data augmentation was broadly performed concerning intensity and spatial.  Intensity augmentation included Bias Field artifacts, Gaussian noise, Gamma, Ghosting effect. In comparison, spatial augmentation consisted of horizontal flipping, vertical flipping, affine transformations, and rotation with a degree of -15 \& 15.


\subsection{Methods for Generating Artificial Anomalies}
\label{sec:Synthetic Datasets}

The datasets used to train the models consisted of medical out-of-distribution (MOOD)  and IXI. All the samples were considered to be healthy with no anomalies. In the absence of test data, 10\% of the data was considered as healthy test cases. Furthermore, we used 20\% of the entire data to create anomalous test cases. The anomalous test set was created synthetically. We used two different approaches to create this data. The first approach included superimposing anomalies on the healthy images. 

The Brats T1 image and its segmented mask were multiplied to extract the anomaly. The result was normalized and reshaped to 256 x 256. The anomaly generated was then finally multiplied with the healthy MOOD+IXI data to obtain the desired test image. Lastly, FAST FSL  has been performed to segment the image. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth] {figs/IXI_brats.jpg}
    \caption{Syntehtic IXI generated using anomaly from BraTs}
    \label{fig:Random}
\end{figure}

The second approach was inspired by \citet{tan2020detecting}.  Each healthy image volume was superimposed with a sphere of altering size and location. We restricted the location towards the center and edges of the brain matter. We further tried to alter intensities for different outlier generations. Lastly, a similar approach was followed with cubical shape outliers. For a given image volume, the following approaches were used to add anomalies to the image. 

\textbf{Random addition}: Spherical anomaly with random intensities is added to the healthy image.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth] {figs/IXI_random.jpg}
    \caption{Random addition on IXI image}
    \label{fig:Random}
\end{figure}


\textbf{Shape deformation}: The intensity of the sphere decreases as you move inwards.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth] {figs/IXI_def.jpg}
    \caption{Shape deformationon IXI image}
    \label{fig:Random}
\end{figure}


\textbf{Copy altered addition}: A spherical copy of the volume is used as a sample which is then shifted by random distance in a random direction.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.45\textwidth] {figs/IXI_alter.jpg}
    \caption{Copy altered addition on IXI image}
    \label{fig:Random}
\end{figure}

==> sections/x_original_eval.tex <==
\section{Experiments and Evaluation}
\label{ch:evaluation}
In this section we explain the results obtained from the different approaches that have been tested to solve the problem of anomaly detection. That would cover all the different convolutional neural networks that have been tested on both the synthetic and BRATS data-set. To simplify the analysis we divide the analysis into three following steps:

\begin{itemize}
  \item Preliminary Experiments
  \item StRegA Experiments
  \item Statistical and Comparative Analysis
\end{itemize}

Preliminary Experiments helped us choose the model with the loss function that is compared against other relevant approaches. We then show the specific experiments relevant to our pipeline in the next section titled StRegA Experiments. To conclude the evaluation we show the statistical performance of our proposed approach to all the other models. As will be seen in the visual results, the data-sets that are used help us in establishing a comprehensive measure on the performance of each approach.

\subsection{Preliminary Experiments}
\label{sec:Preliminary}
In this section we explain all the results obtained from the different Autoencoder and Variational Autoencoder based models that we considered to analyse the performance. To benchmark these results we use the Sørensen–Dice coefficient and Area Under the precision-recall curve (AUPRC) which is a useful metric for imbalanced data. We also cover the various preprocessing and postprocessing steps that are involved in coming up with the pipeline. 

\subsubsection{Comparision of different preprocessing steps}
Before we pass the input image volume to the model for dimensionality reduction followed by reconstruction, we tried several preprocessing steps. 

\paragraph{Clustering as dimensionality reduction}
Another preprocessing step that we attempted as a means of simplifying the data maintaining the structural integrity of the anomaly was to use the different clustering methods to do segmentation of the image slices into 3,4 or 5 classes. After comparing the performance on hierarchical clustering, k-means and the FSL FAST (FMRIB's Automated Segmentation Tool) we noticed that while this approach improved the quality of reconstructions which will be presented in the comparison section, the best approach turned out to be the 4 class FAST segmentation. 

When analysed statistically going over 4 classes did not provide any meaningful improvement in terms of reconstruction as the dice score produced by all the three above classes on our baseline model CeVAE was 0.81 on the synthetic test data-set. This was an improvement over the same model trained over the standard data-set without segmentation where the dice score obtained was 0.77. Thus we utilised this preprocessing on all further models as it provided a meaningful improvement in the quality of reconstruction with lesser amount of detail that is present in the input. 

\subsubsection{Comparision of preliminary model specific experiments}
The initial approach of using the standard dense and spatial autoencoder provided very poor results overall with reconstructions that could not be utilised to detect the anomaly except in very narrow situations. The same situation was true for the standard Variational Autoencoder, where for simple contrast anomalies it was enough to detect the anomaly but in most cases failed to generate an acceptable reconstruction as it was unable to provide proper latent space representation. The Dice score on the BRATS dataset was close to 0.11 and hence we just present here the best case scenario of VAE.
\begin{figure}[h!]
        \centering
        \includegraphics [width=0.459\textwidth] {figs/vae.png}
        \caption{VAE model (a) Input image (b) Reconstruction (c) Anomaly mask} 
        \label{fig: cevae}
\end{figure}
\newline
We then introduced skip connections inspired by \citep{cccc} on both the Dense and Spatial Autoencoders and the Variational autoencoder. While the results on the synthetic data and the MOOD toy test data was better, the more complicated anomalies were harder to detect in the reconstruction. Here we used the combination of L1 distance between the input x and it's reconstruction and the gradient difference loss which forces the model to reconstruct image gradients well. This improved the results significantly in isolating the anomalies but as can be seen in the image below this would still result in very low dice score as it was only detecting the boundary of the anomalies.
\begin{figure}[h!]
        \centering
        \includegraphics [width=0.45\textwidth] {figs/res_skipae.png}
        \caption{SkipAE model (a) Input image (b) Ground Truth (c) Anomaly mask} 
        \label{fig: skipae_res}
\end{figure}
As the anomaly detected on the BRATS in certain specific anomalies like the first case shown above performs well overall the reconstructions on most of the data is again not satisfactory as can be seen in the second example.

Observing the initial approaches it was clear that we needed a better quality of latent space representation and avoid the posterior collapse problem of the VAE based approaches which is where we approached the model Context encoding Variational Autoencoder inspired by \citep{zimmerer2018context}. Utilising the network described in the methodology section we were able to get much better reconstructions on the challenging BRATS data-set. Combining the Context encoding step with the conventional VAE improved the results significantly and the results on the BRATS data-set can be seen in figure \ref{fig: cevae_res}.
\begin{figure}[h!]
        \centering
        \includegraphics [width=0.45\textwidth] {figs/cevae_res.png}
        \caption{CeVAE model (a) Input image (b) Reconstruction (c) Anomaly mask (d) Ground Truth} 
        \label{fig: cevae_res}
\end{figure}

This concludes the preliminary experiments as we felt satisfied with the results of The Dice scores obtained on the CeVAE model for challenging data with pathologies. Though the dice score obtained was still 0.396, it was clear that with using the earlier results of improvement in quality of reconstruction with a simplified input in FAST segmentation, better results could be achieved. This is explained in the next section which involves our novel pipeline for unsupervised anomaly detection. The Dice scores obtained for the preliminary experiments are shown as follows:

\begin{table*}[h!]
  \begin{center}
    \caption{Dice Scores on Preliminary approaches on T2 data}
    \label{tab:table1}
    \begin{tabular}{ |c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\bfseries Model} & 
    \multicolumn{3}{|c|}{\bfseries Dice Score} \\
    \cline{2-4} 
     & MOOD Toy Data & Synthetic Data &  BRATS 2019  \\
    \hline
    Autoencoder (Dense) & 0.321 $\pm$ 0.144 & 0.345 $\pm$ 0.176 & 0.011 $\pm$ 0.113 \\
    \hline
    Autoencoder (Spatial) & 0.179 $\pm$ 0.137 & 0.141 $\pm$ 0.195 & 0.009 $\pm$ 0.097\\
    \hline
    VAE & 0.381 $\pm$ 0.166 & 0.351 $\pm$ 0.126 & 0.134 $\pm$ 0.165\\
    \hline
    SkipAE & 0.517 $\pm$ 0.145 & 0.498 $\pm$ 0.173 & 0.221 $\pm$ 0.101\\
    \hline
    CeVAE & 0.724 $\pm$ 0.145 & 0.712 $\pm$ 0.132 & 0.350 $\pm$ 0.071\\
    \hline
    \end{tabular}
  \end{center}
\end{table*}

The preliminary model experiments comprised of training all the presented models with the baseline hyper parameters and trained on 2D T1 scans of MOOD data-set \footnote{http://medicalood.dkfz.de/web/}. As can be observed in the aforementioned table the results especially on the BRATS data-set were especially poor and were not reliable.

\subsubsection{Preliminary Post-processing approaches}
Preliminary post-processing methods on all baseline models were bench marked with standard difference of the reconstruction with the input volume with manual threshold. However we were unable to reliably maintain a common manual benchmark that allowed to isolate the anomaly as different data-sets required knowledge of the intensity of anomaly that would be detected by a specific model and computing the average over several input data did not yield a satisfactory result. It is clear here that an automated threshold approach such as Otsu or minimum threshold which were eventually used in the final pipeline. To shrink the brighter regions and enlarge the dark regions as a means of isolating the anomaly we used a technique called Morphological erosion which sets a pixel at (i, j) to the minimum over all pixels in the neighbourhood centred at (i, j). Erosion shrinks bright regions and enlarges dark regions. 
\begin{figure}[h!]
        \centering
        \includegraphics [width=0.45\textwidth] {figs/postproc.png}
        \caption{Binary threshold with erosion (a) Input image (b) Reconstruction (c) Anomaly mask (d) Ground Truth} 
        \label{fig: skipae_res}
\end{figure}
\newline
However as can be seen in the above image this results in a lot of additional noise that affects the quality of the anomaly detection. As we approached a model with better quality of reconstruction we later moved to a better pipeline that while using similar ideas of isolating the anomaly, do a much better job with eliminating the remaining noise by using a combination of automatic threshold and Morphological opening which will be presented in the subsequent sections. The initial approach worked to isolate the anomaly but generated too much noise which adversely affected the dice score. The more uniform anomalies like the MOOD Toy test data worked well with this approach as the amount of detail was relatively lower. But in more complex pathology's present in the BRATS data-set this was not usable.

\subsection{StRegA Experiments and Evaluation}
\label{sec:model}
As described in the previous sections the model chosen was CeVAE \citep{zimmerer2018context} which gave the best results in comparison. Using the improved results obtained in the preliminary experiments on FSL FAST 4-class segmented data, we now retrained the CeVAE model with the combination of IXI and MOOD segmented data. When experimenting with the number of layers in the encoder and decoder we noticed that the results on the test data-set i.e. BRATS 2019 improved significantly when we used a more compact model on the segmented data. This could be due to reducing over-fitting on the relatively simpler segmented data. Thus after several experiments, having symmetric 64, 128, 256 feature maps and a latent variable size of 256 yielded the best generalisation in the quality of reconstruction. This as mentioned in the methodology section, we term as Compact Context-Encoding Variational Autoencoder (cceVAE) that is a part of our pipeline along with the input 4-class segmented images. We also established that having more data in the form of modalities i.e. T1, T2 and Proton Density images as training data to help as regularisation. We noticed that the standard ceVAE model when trained with the combination of the three modalities approached a dice score of 0.44 on the BRATS data-set when trained with segmented T1, T2 and PD volumes as compared to training on just T2 volumes where the reported dice score was 0.40 when tested on T2 data. Implementing skip connections as was used in earlier mentioned model SkipAE provided no meaningful improvements but residual connections with batch normalisation provided marginal improvements and were thus included in the model. 
Thus the final pipeline is as follows:
\begin{itemize}
  \item Input volume Segmentation with FSL FAST
  \item Min-max normalisation
  \item Passed through Compact Context-Encoding Variational Autoencoder (cceVAE)
  \item Difference of reconstruction and input to model
  \item Otsu thresholding
  \item Morphological opening -> \textbf{Final output}
\end{itemize}

\subsubsection{Pipeline}
Here we present the visual results of the pipeline in detail. As mentioned before here we can see the steps in progression of the pipeline to get the detection of anomaly in the brain.
\begin{figure*}[h!]
        \centering
        \includegraphics [width=\textwidth] {figs/t1-final.png}
        \caption{StRegA results on BRATS dataset (T1) images (a) Input Image (b) Segmented Image (c) Reconstruction (d) Manual and Otsu thresholding (e) Morphological Opening -> \textbf{Final prediction} (f) Ground Truth} 
        \label{fig: t1-final}
\end{figure*}

For a challenging test case, we provide the results obtained on the BRATS dataset as mentioned before which is data with pathology and thus interesting in practical applications.

\begin{figure*}[h!]
        \centering
        \includegraphics [width=\textwidth] {figs/t2-final.png}
        \caption{StRegA results on BRATS dataset (T2) images (a) Input Image (b) Segmented Image (c) Reconstruction (d) Manual and Otsu thresholding (e) Morphological Opening -> \textbf{Final prediction} (f) Ground Truth} 
        \label{fig: t2-final}
\end{figure*}

\begin{figure*}[h!]
        \centering
        \includegraphics [width=\textwidth] {figs/syn_pipeline.png}
        \caption{StRegA results on synthetically generated data} 
        \label{fig: syn-final}
\end{figure*}

As can be inferred from the above pipeline, one immediate point of concern is the size of anomaly in the input image. As morphological opening would eliminate the prediction if it is too small. So for anomalies that are much smaller it would be good to reduce the area threshold. But over several different kinds and shapes of anomalies that we generated synthetically, the results were better in comparison with the other models. Figure \ref{fig: syn-final} shows the pipeline for synthetic data where for more uniform anomalies the model is able to segment them almost perfectly.

\subsection{Statistical and Comparative Results}
\label{sec:comparison}
\subsubsection{Statistical Significance}
Our proposed pipeline provides a big improvement in anomaly detection as compared to the relevant models that were tested and also a significant improvement over the model which we started with i.e. CeVAE. To show that these results are statistically significant we perform a t-test over the results of the two approaches i.e the baseline CeVAE and our proposed pipeline StRegA. Essentially a t-test allows us to compare the average values of the two data sets and determine if they came from the same population. Mathematically t-test takes a sample from each of the two sets and establishes the problem statement by assuming a null hypothesis that the two means are equal. If the null hypothesis is to be rejected, then it indicates that the data readings are statistically significant. As we finalised the best model as baseline being CeVAE and comparing our final pipeline, we have a P value of 7.36e-13 which voids the null hypothesis and says that the difference is statistically significant. 

\subsubsection{Comparative Analysis}
Here we present the comparison of our pipeline with the baseline that we started with which was CeVAE \citep{zimmerer2018context} trained similarly on the T1, T2 and PD volumes from IXI and MOOD data-sets. We then compare and contrast our model also with Bayesian Skip Autoencoder \citep{cccc} and Gaussian Mixture Variational Autoencoder \citep{chen2020unsupervised}.
\begin{figure*}[h!]
        \centering
        \includegraphics [width=\textwidth] {figs/compare_analysis.png}
        \caption{Comparative results from different methods. Top row: artificially generated anomalous data. Bottom row: BraTS T2w image. (a) A slice from the input volume, (b) ceVAE, (c) SkipVAE, (d) GMVAE, (e) StRegA and (f) ground truth} 
        \label{fig: compare_res}
\end{figure*}
Both qualitative and quantitative analysis are performed on the three data-sets ref. MOOD Toy data, Synthetically generated data as mentioned in earlier section and BRATS. The input image and final predictions are shown visually for all the aforementioned models to compare the quality of prediction of the anomaly in figure \ref{fig: compare_res}.
Following are the Dice scores of the final model in comparison with the baseline and other models that were tested.
\pagebreak
\begin{table*}[h!]
  \begin{center}
    \caption{Comparitive results of StRegA with other models on T1 data.}
    \label{tab:table1}
    \begin{tabular}{ |c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\bfseries Model} & 
    \multicolumn{3}{|c|}{\bfseries Dice Score ($\mu\pm\sigma$)} \\
    \cline{2-4} 
     & MOOD Toy Data & Synthetic Anomalous Data &  BRATS  \\
    \hline
    SkipAE & 0.443 $\pm$ 0.136 & 0.498 $\pm$ 0.164 & 0.209 $\pm$ 0.113\\
    \hline
    GMVAE & 0.657 $\pm$ 0.121 & 0.711 $\pm$ 0.105 & 0.337 $\pm$ 0.124\\
    \hline
     ceVAE & 0.633 $\pm$ 0.145 & 0.690 $\pm$ 0.164 & 0.356 $\pm$ 0.132\\
    \hline
     ceVAE (with StRegA pre-processing) & 0.724 $\pm$ 0.132 & 0.710 $\pm$ 0.111 & 0.520 $\pm$ 0.108\\
    \hline
    \textbf{StRegA}  & 0.737 $\pm$ 0.098 & 0.723 $\pm$ 0.134 & 0.531 $\pm$ 0.112\\
    \hline
    \end{tabular}
  \end{center}
\end{table*}

\begin{table*}[h!]
  \begin{center}
    \caption{Comparitive results of StRegA with other models on T2 data.}
    \label{tab:table1}
    \begin{tabular}{ |c|c|c|c|c|}
    \hline
    \multirow{2}{*}{\bfseries Model} & 
    \multicolumn{3}{|c|}{\bfseries Dice Score ($\mu\pm\sigma$)} \\
    \cline{2-4} 
     & MOOD Toy Data & Synthetic Anomalous Data &  BRATS  \\
    \hline
    SkipAE & 0.517 $\pm$ 0.145 & 0.498 $\pm$ 0.173 & 0.221 $\pm$ 0.101\\
    \hline
    GMVAE & 0.699 $\pm$ 0.121 & 0.701 $\pm$ 0.121 & 0.340 $\pm$ 0.167\\
    \hline
     ceVAE & 0.724 $\pm$ 0.145 & 0.712 $\pm$ 0.132 & 0.350 $\pm$ 0.071\\
    \hline
     ceVAE (with StRegA pre-processing) & 0.797 $\pm$ 0.099 & 0.783 $\pm$ 0.111 & 0.522 $\pm$ 0.135\\
    \hline
    \textbf{StRegA}  & 0.856 $\pm$ 0.098 & 0.859 $\pm$ 0.112 & 0.642 $\pm$ 0.101\\
    \hline
    \end{tabular}
  \end{center}
\end{table*}

\begin{figure}[h!]
        \centering
        \includegraphics [width=0.45\textwidth] {figs/violin.png}
        \caption{Violin plot comparing predictions on BRATS T2 data} 
        \label{fig: compare_res}
\end{figure}




==> sections/x_original_relatedwork.tex <==
\subsection{Related Work}
\label{ch:relatedwork}

Reconstruction errors are commonly used in unsupervised anomaly detection, acknowledging the regular distribution models cannot effectively reproduce anomalies. Therefore, regular data is distinguishable from anomalous data with the degree of error differences. The majority of the methods assume losses are optimised for average distribution data, whereas anomalies are impacted with significant losses when their dimensions are reduced. In recent times, unsupervised and deep learning methods have derived state-of-the-art models for approximating high-dimensional imaging data.  

Generative Adversarial Networks (GAN) \citep{goodfellow2014generative} and Variational Auto-Encoder (VAE) \citep{kingma2019introduction}  are two essential methods based on latent variable modelling.  However, both these methods have individual approaches for the distribution. VAE  applies variational inference to approximate the data distribution. The posterior distribution is encoded into latent space using the encoder network of the VAE, whereas the decoder network is responsible for modelling the likelihood. Unlike VAE, the generator network of the GAN converts the prior distribution of the random samples in the latent space to data samples that an optimised classifier cannot distinguish. The obtained data distribution is infer-able, and GAN is mainly a sampler. Recently some researchers \citep{carrara2021combining} have coupled an autoencoder with GAN to derive enhanced latent representations in the domain of anomaly detection. 


\subsubsection{Variational Autoencoder (VAE)}

% cite the paper here in the name.% cite the paper here in the name.
Variational Auto encoders (\cite{zimmerer2019unsupervised}) belong to a class of generative models that provides a probabilistic way to represent the observations in the latent space. Unlike an Autoencoder, the encoder of the Variational Autoencoder describes the probability distribution of each latent attribute. The architecture of the network is a 5-layer fully convolutional encoder and decoder. During training, the model computes a Latent Space Representation (LSR) of the non-anomalous input image, thus learning the feature distribution of a healthy dataset. The latent space in VAEs is continuous by design and allows easy random sampling and interpolation. This is achieved by designing the encoder to output two vectors:  a vector of means $\mu$ of data samples and a vector of standard deviations $\sigma$. The encoding are generated within these distributions, and the decoder learns that not just a single point but all the points around it are referred to as a sample of the same class, thus decoding even slight variations of the encoding. In our work, the network is trained by optimising the evidence lower bound (ELBO) 'L', which can be defined as:

\begin{equation}
\log p(x) \geq L=-D_{K L}(q(z \mid x) \| p(z))+E_{q(z \mid x)}[\log p(x \mid z)]
\end{equation}
where, q(z$\mid$ x) and  p(x$\mid$ z) are diagonal normal distributions that are parameterized by neural networks $f_\mu$, $f_\sigma$, and $g_\mu$, and constant c such that:

\begin{equation}
\mathrm{q}(\mathrm{z} \mid x)=N\left(z ; f_{\mu, \theta 1}(x), f_{\sigma, \theta 2}(x)^{2}\right)
\end{equation}
\begin{equation}
p(x \mid z)=N\left(x ; g_{\mu, \gamma}(z), I * c\right)
\end{equation}
 
\subsubsection{Scale-Space Autoencoder}

There exist many variations of auto encoders that have been proposed.One of them is  \textbf{Scale-Space Autoencoder} \citep{baur2020scalespace} .This framework is used for unsupervised anomaly detection based on the Laplacian Pyramid, allowing efficient compression and reconstruction of brain MRI images with high fidelity and successfully suppressing anomalies. Contrary to other frameworks, this framework models the distribution of the scale-space representation of healthy brain MRI. The Laplacian pyramid is a multi-scale representation of the input image; it allows efficient segmentation of anomalies at different resolutions and then aggregates the results. SSAE architecture is an encoder-decoder network that aims to localise anomalies from reconstruction residuals. The frequency band of the input data is split by compressing and reconstructing the Laplacian pyramid of the healthy brain MRI. To obtain a Laplacian pyramid with K levels, the input image x is repeatedly smoothed and down sampled. Reconstruction can be recursively determined using
\begin{equation}
   \hat{x} = \sum_{k=0}^{K-1} u(I_{K-k}) + H_{K-1-k}
\end{equation}
where $I_k$ is the low-resolution representation of the image x after K down samplings and high-frequency residuals $H_0,..,H_{K-1}$ which are obtained at each level k using :
\begin{equation}
   H_k = I_k - u(I_{k+1}) ; \forall 0	\leq k<K
\end{equation}
The overall loss can be defined as the weighted sum of losses at all scales:
\begin{equation}
   L = \sum_{k=0}^{K} \lambda_kL_k
\end{equation}
where,
\begin{equation}
   L_k = l2(I_k, \hat{I_k}) = l2(I_k, u(\hat{I_k}+\hat{H_k})
\end{equation}


\subsubsection{Bayesian Skip Auto encoder}
Bayesian Skip  Auto encoder  \citep{cccc}  is formulated on a concept that has been used and proven advantageous for biomedical image segmentation.  This framework makes use of skip connections that allow the models with limited capacity to be trained and used for unsupervised anomaly detection. Skip connections in Auto encoders facilitate the reconstruction of high resolution and complex medical data with high fidelity. A drop-out-based identity mitigation technique is employed to prevent the model from learning an identity mapping and allowing it to bypass the lower levels of the Auto encoder. The loss function for the model can be defined as:
 \begin{equation}
   L(x, \hat{x}) = l_1(x, \hat{x}) _ gdl(x, \hat{x})
\end{equation}
Here,’l1’  is defined as the ‘l1’-distance between the input and its reconstruction x and $\hat{x}$ respectively, gdl(.,.) is the gradient difference loss.


\subsubsection{Vector  Quantized  Variational  Auto encoder}

Vector  Quantized  Variational  Auto encoder  \citep{marimont2020anomaly} framework encodes the images in categorical latent space. Further, an Auto-Regressive(AR) model is used to model the prior distribution of latent codes. The prior probability approximated by the AR model is then used for unsupervised anomaly detection and gives the sample and pixel-wise anomaly scores. The encoder of the VQVAE framework is based on a dictionary mapping K discrete keys into a D-dimensional embedding space, i.e., observed variables are mapped to the embedding space, $z_e(x) \in R^D$. The posterior in VQVAE is defined as :
\begin{equation}
    q(z = k \mid x) = 
    \begin{cases}
            1, & for k = \operatorname*{arg\,min}_j || z_e(x) - e_j ||_2\\
    0, & \text{otherwise}
    \end{cases}
\end{equation}
The embedding in the dictionary that is nearest to the output of the encoder is given to the decoder as an input, i.e.,$z_q(x) \sim q(z\mid x)$. The decoder then reconstructs the distribution $p(x\mid z_q(x))$.The VQVAE Loss function is therefore defined as:
\begin{equation}
  L = log(x\mid z_q(x)) + \mid\mid sg[z_e(x)]-e\mid\mid_2^2 + \mid\mid sg[e] - z_e(x)\mid\mid_2^2  
\end{equation}
where, sg[.] is the stop gradient operator.
Further, An Auto-Regressive model is employed to learn the prior distribution of VQVAE, and the probability of samples is approximated. The samples with low probability are identified as anomalies. AR models generate multiple restorations as they are generative models and allow sampling of one variable at a time in an iterative manner. 

\subsubsection{Deep Autoencoders}

Deep auto-encoders employ deep generative representation learning to learn the distribution of a healthy brain anatomy. This understanding should help the model to fully reconstruct healthy brain anatomy although failing to reconstruct anomalous lesions in images of a diseased brain. The model is adopted from  VAEGAN \citep{yu2019vaegan}. The parameter mapping from input $x \in R^{H x W}$, to a lower dimensional representation $z \in R^{d}$ and eventually decoding back to high reconstruction  $ \hat{a}  \in R^{H x W}$ encoder and decoder. The framework is optimised using two loss functions. The VAE component of the model is optimised using 

   \begin{equation}
L_{V A E}=\lambda_{1} L_{r e c}+\lambda_{2} L_{p r i o r}+\lambda_{3} L_{a d v}
\end{equation}
   
   while the discriminator is trained similarly to GAN framework:
   
   \begin{equation}
L_{D i s}=-\log (D i s(x))-\log (1-D i s(D e c(\operatorname{Enc}(x))))
\end{equation}
   
The process of detecting anomalies involve 1. computing the l1 distance between input and reconstruction image, and 
2. threshold the resulting residual image to obtain a binary segmentation.


\subsubsection{Gaussian  Mixture  Variational  Autoencoder}
The Gaussian  Mixture  Variational  Auto encoder \citep{chen2020unsupervised}  approach (GMVAE) combines image restoration techniques with unsupervised learning based on  Deep  Learning.   A GMVAE is first trained on healthy subjects to learn a normative prior distribution. A Maximum-A-Posteriori (MAP) restoration model then makes use of this prior to detect the outliers. In GMVAE, the ELBO is formally expressed as:
    
    $ \mathbb{E}{q(z\mid X)} [log p(X\mid z)] - \mathbb{E}{q(\omega \mid X) p(c \mid z, \omega)} [KL [q(z \mid X) | p(z \mid \omega, c)]]$\\
            $ - [KL [q(\omega \mid X) | p(\omega)]] - \mathbb{E}_{q(z \mid X) q(\omega \mid X)} [KL [p(c \mid z, \omega) | p(c)]]$
            
Where the first part is the reconstruction term, the second part ensures the encoder distribution fits the prior, the third term does not let the posterior $\omega$ diverge from the prior $p(\omega)$, and the last term enforces the model to not collapse into a single gaussian but uses the mixture model. For the architectural choice, seven convolutional layers for the encoder and seven transpose layers for the decoder are used. The latent variables z and $\omega$ are 2D structures with size (32, 42 1) and nine clusters, c.

\subsubsection{Adversarial autoencoder}
Adversarial auto encoder \citep{makhzani2016adversarial} converts an auto encoder into a generative model. The objective is two-fold - a regular reconstruction loss and an adversarial training loss. The second loss criterion tends to match the aggregated posterior distribution of the latent space of auto encoder to an arbitrary prior distribution. An outcome of this architecture bounds the encoder module to learn the data distribution close to the prior distribution, and the decoder maps the imposed prior to the data distribution. The encoding function of the encoder is formally represented as 
\begin{equation} 
q(z) = \int_x q(z\mid x) p_d(x) dx 
\end{equation} 
where, x is the input and z is its latent representation vector. $p(z)$ be the prior distribution to be imposed on the latent vectors,$q(z|x)$ is an encoding dimension, and p(x$\mid$ z) is the decoding distribution. Also, $p_d(x)$ is the data distribution and p(x) is the model distribution. The adversarial auto encoder is regularised by matching this aggregated posterior q(z), to an arbitrary prior, p(z). The whole training takes place in two phases - \emph{reconstruction} phase where the encoder and decoder are updated to minimise the reconstruction error in the input. Later in the \emph{regularisation} phase, the adversarial network updates the discriminator to classify better actual samples (from the prior) from the generated samples (from the encoder). Finally, the generator or the encoder is updated to confuse the discriminator. Thus we have three different optimisations in the whole pipeline.


\subsubsection{Constrained Adversarial Auto encoder}
Constrained Adversarial Auto encoder \citep{chen2018unsupervised}, addresses the limitation of existing methods that lack consistency in latent representations by an effective constraint that helps map an image with a lesion close to its corresponding healthy image in the latent space. Given a set of healthy images $X_h \in R^{d x d}$, a model is trained to learn a distribution $P(X_h) = \int P (X_h \mid z) P(z) dz$. Once $P(X_h)$ is obtained,  images with lesions (abnormal regions) are fed into the models. As these models were trained only on healthy images they do not reconstruct accurately and are further detected by pixel-wise intensity difference of the original and reconstructed counterparts. In this approach the GAN module of Adversarial auto encoders (AAE) is replaced with Wasserstein GAN with gradient penalty (WGAN-GP) and is mathematically expressed as: 

\begin{equation}
    \min_G \max_D [ E_{z \sim q(z \mid X)} D(z) - E _{z_{prior} \sim p(z)} D(z_{prior})] + \lambda E_{z \sim q(z \mid X)} [(|| \nabla_z (D(z)) ||_2 - 1)^2]
\end{equation}

For the decoder unit, $p(X_h \mid z) \sim \mathcal{N} (X; \mu(z \mid X_h), \textbf{I})$ is assumed and $L_2$ loss is selected as the reconstruction loss $|| X - X^\prime||_2$. Further the objectives of VAE and AAE are generalised as, $L_{auto-encoder} + L_{divergence}$. In the end a ResNet structure is used for the encoder and decoder module. 


==> sections/x_quasioriginal_method.tex <==

\section{Methodology}
\label{ch:methods}


\subsection{StRegA : Segmentation Regularised Anomaly }
The proposed unsupervised anomaly detection pipeline, StRegA: Segmentation Regularised Anomaly - shown in Fig.\ref{fig:StRegA}, includes a modified compact version of the Context-encoding Variational Autoencoder (ceVAE) \citep{zimmerer2018context} - Compact ceVAE (cceVAE), combined with pre and post-processing steps. Anomaly detection is performed in 2D, per-slice basis. The input volumes are pre-processed in 3D, then slices are supplied to the model, followed by that, post-processing steps are applied, and finally, the slices are stacked together to obtain the final result in 3D. 

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.9\textwidth] {figs/strega.png}
    \caption{StRegA pipeline.} 
    \label{fig:StRegA}
\end{figure*}

\subsubsection{Preprocessing}
\label{sec:Preprocessing}
The first pre-processing step was to segment the input image into different tissue types and obtain the corresponding segmentation mask. Segmentation means partitioning the input images into various segments. Segmentation can simplify the input given to the model, consequently improving the performance of the anomaly detection system. This was performed by supplying the 3D brain images to automatic segmentation tool of FSL (\cite{jenkinson2012fsl}) - FAST, which segmented the brain into three different tissue types: grey matter, white matter, cerebrospinal fluid (CSF); and background - a total of four classes. The underlying principle of FAST is formulated on a hidden Markov random field model and an associated expectation-maximisation algorithm. The entire process is automated and is capable of producing a probabilistic/partial volume tissue segmentation. Apart from segmenting the input volume, this tool also corrects for spatial intensity variations (also known as bias field or RF inhomogeneities). The segmentation mask was normalised and standardised with the intensity distribution of the dataset - normalised with zero mean and unit variance. The volumes were divided into 2D slices and then they were resized to 256×256 in-plane using bilinear interpolation before feeding them into the network. During the training phase, in addition to the above mentioned pre-processing steps, data augmentation was also performed. The augmentation techniques used can be grouped into two groups: intensity-based and spatial augmentation. Intensity augmentation included bias field artefacts, Gaussian noise,  random gamma, and ghosting artefacts. While spatial augmentation consisted of horizontal flipping, vertical flipping, affine transformations, and rotation with a degree between -15 and +15.

%\begin{figure}[H]
%    \centering
%    \includegraphics[width=0.45\textwidth] %{figs/preprocess.png}
%    \caption{FSL FAST Segmentation}
%    \label{fig:preprocess}
%\end{figure}


%\begin{figure*}
%    \centering
%    \includegraphics[width=0.9\textwidth] %{figs/Preprocess_BD.png}
%    \caption{Pre-processing}
%    \label{fig:Preprocess_BD}
%\end{figure*}

\subsubsection{Network Model: cceVAE}
\label{sec:model}
This work proposes a compact modified version of the ceVAE model \citep{zimmerer2018context}, explained in Sec.\ref{sec:ceVAE}: Compact ceVAE(ccVAE). This is a compact version as it has smaller encoder and decoder than the original ceVAE - having symmetric encoder-decoder with 64, 128, 256 feature maps, and a latent variable size of 256. This proposed model also uses residual connections and batch normalisation layers - which were not present in ceVAE. The preprocessed images are fed into this network model and network tries to reconstruct the input. During training, anomaly-free (in the experiments of this paper: healthy brain MRIs) images are provided and the network attempts to learn a Gaussian distribution of the given anomaly-free dataset. While inference, the network attempts to reconstruct the input image from the learnt Gaussian distribution. If the network encounters images with anomalies - they are then out-of-distribution samples. Hence, the network should "in-theory" fail to reconstruct the anomalies as they do not belong to the learnt distribution. The reconstruction difference is then computed by subtracting the model's output from its input to generate the initial anomaly mask - which is then post-processed to finally detect the anomaly.


\subsubsection{Postprocessing}
\label{sec:Postprocessing}
After subtracting the reconstruction from the model's input, the initial mask is obtained. The mask is first thresholded to eliminate any pixel having a value less than zero, by replacing all the negative values with zero. Then to remove the intensity outliers, the mask was thresholded using Otsu's method \footnote{\url{https://en.wikipedia.org/wiki/Otsu's_method}}. This is a frequently used method for performing automatic image thresholding which divides all the pixels into two classes - background and foreground, based on a single intensity threshold. The threshold is calculated by minimising intra-class intensity variance, or in other words, by maximising inter-class variance. \footnote{\url{http://www.labbookpages.co.uk/software/imgProc/otsuThreshold.html}}. After performing Otsu thresholding, the small irrelevant parts of the mask is removed by applying morphological opening \footnote{\url{https://en.wikipedia.org/wiki/Opening_(morphology)}} - which removes all bright structures of an image with a surface smaller than the area threshold. It is equivalent to applying dilation on top of erosion on the image. This gives the final anomaly mask. It is then resized through interpolation to whichever input size the original image had before resizing during preprocessing. Finally, all the slice-wise 2D masks are stacked together to get the final anomaly mask in 3D.

%\begin{figure*}[h!]
%    \centering
%    \includegraphics[width=0.9\textwidth] %{figs/postprocess_BD.png}
%    \caption{Post-processing} 
%    \label{fig:postprocess_BD}
%\end{figure*}


\subsection{Datasets}
\label{sec:Datasets}
Training unsupervised anomaly detection models warrants for anomaly-free datasets. As the focus of this paper is on brain MRIs, two anomaly-free datasets were selected for training the models: MOOD challenge dataset \citep{mood_2021_4573948} and IXI dataset \footnote{IXI Dataset: \url{ https://brain-development.org/ixi-dataset/}}. It is worth mentioning that even though both the datasets contain MRIs only from normal, healthy subjects - there might still be some anomalies present in some of the MRIs which were missed by the experts. However, in this research, following the authors of the datasets - these datasets were considered to be comprising of only anomaly-free healthy brain MRIs. MOOD dataset comprises of 800 T1w brain MRIs with matrix size of 256x256x256 - 700 of which were used for trainning and 100 were held-out for testing, while the IXI dataset contains MRIs of nearly 600 subjects - all of which were used in training, acquired using 1.5T and 3T MRIs in three different hospitals, with different MRI sequences: T1w, T2w, PDw, MRA, and DTI. In this research, T1w and T2w images from the IXI dataset were used separately - for training separate T1 and T2 models. Trainings were performed by combining MOOD with one of the IXI contrast: MOOD+IXIT1 and MOOD+IXIT2. 

For evaluating the approach with a dataset with clinical anomalies, 80 randomly selected volumes from BraTS 2017 \footnote{BraTs: \url{https://www.med.upenn.edu/sbia/brats2017/data.html}} dataset was used, which contains four types MRIs with high and low-grade brain tumours: T1-weighted, and contrast enhanced T1-weighted (with contrast agent), T2-FLAIR, and T2-weighted. In this paper, contrast enhanced T1-weighted (T1ce) and T2-weighted MRIs were used. Additionally, the model was also tested on the "toy testset" provided in the MOOD dataset, comprising of one anomaly-free and three anomalous MRIs containing artificial anomalies. It is noteworthy that the image contrasts, acquisition parameters, and other image properties of the BraTS dataset is very different from the training sets. Hence, a controlled synthetic anomalous dataset was created as a part of this research - to evaluate the approach on a dataset which contains anomalies, but the contrast and other image characteristics are similar to the training set. Methods used to generate different types of artificial anomalies for creating this synthetic anomalous dataset are explained in the following section.

\subsection{Generating Artificial Anomalies}
\label{sec:Synthetic_Datasets}

Our proposed model was trained on combining two data sets, namely medical out-of-distribution (MOOD) and IXI datasets. Section 3 explains these datasets in detail.  Both these datasets consist of healthy brain volumes with no anomalies.  In the absence of anomalous test data, 10\% of the input data was considered as healthy test cases. Furthermore, we used 20\% of the entire data to create anomalous test cases. The anomalous test set was created synthetically. 

% Our first approach was inspired by Neural style transfer\citep{jing2018neural}, a deep learning technique for composing new images by inheriting the style of another image. Neural style transfer is an optimization technique. These techniques use three images, a content image, a style reference image, and the input image you want to style. The model blends them in such a way that the input image is modified with the style of the style reference image. In our scenario, we used the BRATS image as style since it consisted of the anomaly data, and the MOOD image was used as the content image. Our goal here was to transfer the anomaly from BRATS data (style image) to our input data. Referring to figure \ref{fig:nst} , we notice that the contrast of BRATS was transferred to our MOOD image rather than just the anomaly. Though we find great use cases for this method, currently Neural style transfer could not be used for generating anomalous data. However, Neural style transfer could be used to generate similar image volumes of varying intensities, which is out of the scope of our current research. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.45\textwidth] {figs/NST.png}
%     \caption{Neural Style Transfer with MOOD data as input and BRATS image as style.}
%     \label{fig:nst}
% \end{figure}


% Following our learnings from the previous experiments, we adopted two different approaches to creating anomalous data. 
% The two approaches as discussed below provided us with anomalous test data that could be used to test our models. 


\subsubsection{Superimposing BRATS Anomaly}
\label{sec:Superimposing BRATS Anomaly}


The approach included superimposing anomalies on the healthy images. We first consider an anomalous Brats T1 image along with its label.  The idea is to superimpose BRATS anomalous part on healthy image data. To acquire this, we first multiply the BRATS T1 image and its segmented mask to extract the anomaly. The generated mask can now be used with other healthy data set. In order to do so, we first normalise the mask to clamp the values between 0 and 1, and then reshape the generated mask to 256 x 256. The anomaly generated can then finally be added to the healthy MOOD data to obtain the desired test image. This arithmetic operation adds the anomaly from BRATS TI image at the same location on the healthy images of the MOOD dataset.  Lastly, FAST FSL has been performed to segment the image. The segmented image can be used as an input for testing the model. Consider a BRATS image sample B and it's corresponding segmented mask S, the superimposed MOOD image sample A of patch h can be calculated as :



\begin{equation}
  \begin{array}{l}
    A'_{i} = A_{i} + M_{i} ; \forall i \in h \text{ ,where }    \\ \cr
     M_{j} = B_{j} - S_{j} ; \forall j \in h
  \end{array}
\end{equation}

% Figure \ref{fig: syn} shows various IXI datasets with synthetically generated anomalies. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth] {figs/MOOD_brats.png}
    \caption{Synthetic MOOD image generated using anomaly from BRATS data set}
    \label{fig: syn}
\end{figure}

% \subsubsection{Synthetic Generation of Anomaly}
% \label{sec:Synethtical Generation of Anomaly}
% The second approach, inspired by \citet{tan2020detecting} allows us to introduce anomalies of different shapes and sizes. The procedure was carried out by synthetically generating anomalous data and superimposing it to healthy brain volume. Each healthy image volume was superimposed with a sphere or rectangle of altering size and location. The location ad intensity were the two crucial elements of superimposing this anomaly. the location determined where the anomaly would be situated, where the intensity reflected how bright the anomaly would be. Both these factors defined the realisation of anomaly. We restricted the location of superimposing towards the center and edges of the brain matter. The anomaly location should be as realistic as an actual anomaly. We further tried to alter intensities for different outlier generations. Lastly, a similar approach was followed with cubical shape outliers. Finally, to create anomalous image volume, we synthesise five types of generation based on location or intensity.  The performance of the generated anomaly is measured using a dice score. 

% Following are five types of anomalous mask generating methods. All of these approaches differ in terms of location, intensity, and shape of anomaly. 

% \textbf{Unvaried addition}: A spherical anomaly is generated with uniform intensities and is added to a healthy image volume at a random location.  For an image sample I, with patch h and i is the pixel information of patch h, we can formulate random addition as:
% \begin{equation}
%     I'_{i} = I_{i} + n ; \forall i \in h,\text{ where } n \sim \mathcal{N} (0,1)
% \end{equation}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.45\textwidth] {figs/anomaly.png}
%     \caption{Synthetic generated data volume using IXI dataset, from above they are Unvaried addition, Symmetric Parallel Addition, Copy altered addition, Random addition and Shape deformation }
%     \label{fig: syn}
% \end{figure}

% \textbf{Random addition}: A spherical anomaly is generated with random intensities and is added to a healthy image volume at a random location.  For an image sample I, with patch h and i is the pixel information of patch h, we can formulate random addition as:

% \begin{equation}
%     I'_{i} = I_{i} + n ; \forall i \in h, \text{ where } n \sim \mathcal{N} (0,1)
% \end{equation}


% \textbf{Shape deformation}: The anomalous mask is generated as a sphere and the pixels are shifted away from the center of the sphere. For an image sample I, with patch h and A as the 3-dimensional coordinates of a pixel in patch h with s as the centre of the sphere, we can formulate shape deformation as : 

% \begin{equation}
%   \begin{array}{l}
%     I'_{A} = I_{v} ; \forall A \in h, A = (i,j,k) \text{ and.}    \\ \cr
%      V = h'_{c} + s(A - h'_{c}) 
%   \end{array}
% \end{equation}


% \textbf{Copy altered addition}: This type of anomaly is generated by considering a spherical portion of the healthy brain. The spherical copy of the volume is used as a base sample. This sample is then altered by shifting random distance in a random direction. For an image sample I, with patch h and I as the 3-dimensional coordinates of a pixel in patch h, we can formulate shape deformation as : 

% \begin{equation}
%   \begin{array}{l}
%     I'_{a,b,c} = I_{a+i ,b+j , c+k} ; \forall a,b,c\in h, \\ \cr
%     \text { where } i,j,k \sim \sigma \mu (0.03 \cdot d , 0.06 \cdot d)  \\ \cr
%     \text{ and }  \sigma  =
%     \begin{cases}
%             +1, \text{with probability 0.5}\\
%             -1, \text{with probability 0.5}
%     \end{cases}  \\ 
%   \end{array}
% \end{equation}


% \textbf{Symmetric Parallel Addition}:  The anomalous image volume is generated by re sampling a spherical portion of the healthy brain just like in the case of copy alteration addition. however, the main difference here is the sample is reflected along the axis of symmetry and no random alterations are done in the pixels. For an image sample I, with patch h and (a,b,c) as the 3-dimensional coordinates of a pixel in patch h, we can formulate shape deformation as :

% \begin{equation}
%     \begin{array}{l}
%         I'_{a,b,c} = I_{a, d-b , c}  \forall a,b,c \in h, \\ \cr
%         \text{ where d is the image width } 
%   \end{array}  
% \end{equation}


